The design of the Ali CMB Polarization Telescope receiver

Ali CMB Polarization Telescope (AliCPT-1) is the first CMB degree-scale polarimeter to be deployed on the Tibetan plateau at 5,250m above sea level. AliCPT-1 is a 90/150 GHz 72 cm aperture, two-lens refracting telescope cooled down to 4 K. Alumina lenses, 800mm in diameter, image the CMB in a 33.4{\deg} field of view on a 636mm wide focal plane. The modularized focal plane consists of dichroic polarization-sensitive Transition-Edge Sensors (TESes). Each module includes 1,704 optically active TESes fabricated on a 150mm diameter silicon wafer. Each TES array is read out with a microwave multiplexing readout system capable of a multiplexing factor up to 2,048. Such a large multiplexing factor has allowed the practical deployment of tens of thousands of detectors, enabling the design of a receiver that can operate up to 19 TES arrays for a total of 32,376 TESes. AliCPT-1 leverages the technological advancements in the detector design from multiple generations of previously successful feedhorn-coupled polarimeters, and in the instrument design from BICEP-3, but applied on a larger scale. The cryostat receiver is currently under integration and testing. During the first deployment year, the focal plane will be populated with up to 4 TES arrays. Further TES arrays will be deployed in the following years, fully populating the focal plane with 19 arrays on the fourth deployment year. Here we present the AliCPT-1 receiver design, and how the design has been optimized to meet the experimental requirements.

==> Readout_Chain.tex <==
A set of RF and DC lines are required to successfully read out the $\mu$mux resonators of each detector module.  A wider overview of this setup can be found in this AliCPT-1 paper\cite{Salatino20}. Various coaxial cables and microwave components are employed to deliver probe tones from room temperature electronics to the $mu$mux resonators at the focal plane and back.  Careful consideration was given to reach the optimum power of roughly -70 dBm at the $\mu$mux resonators while minimizing the noise temperature and thermal contributions.  Figure~\ref{fig:CryoRF_Chain} shows the latest cryogenic RF chain calculation for this process.  Stainless steel coax of 2.19mm outer diameter is used down to 4K, afterwards switching to 0.86mm stainless steel on the input to the detectors and 0.86mm superconducting NbTi coax on the output up to 4K.  Attenuators and LNAs are also included to correctly model the expected power level at all stages.  The circulator, DC blocks, and (isothermal) copper coax in the RF chain are not included in these calculations, as they have a minimal contribution to attenuation in the system.

\begin{figure}
\begin{center}
\includegraphics[width=1.\textwidth]{figure/Readout_Chain/Test.png}
\end{center}
\caption{
{\color{orange}From Jeremy: I'm aware diagram font is a bit small to read.  Trying to figuring out way to format it better.}
The latest cryogenic RF chain calculations for the readout of the $\mu$mux resonators.  Components included have listed values for input power (S), temperature (T), attenuation (A) or gain (G), output power (P), cascaded noise temperature (T\_casc), noise temperature up to each component (T\_N), cable length, and power dissipated thermally or via attenuation (assuming 2000 probe tones for one RF chain).  Note: the LNA temperatures listed are their conservative noise temperatures.  Some aspects, such as attenuator values and cable lengths, might still be adjusted between now and the first on-sky measurements.}\label{fig:CryoRF_Chain}
\end{figure}

There will be 4 identical readout feedthrough panels into the cryostat (Fig.~\ref{fig:Readout_Feedthrough}), each capable of reading up to 5 final detector modules.  This entails 10x coaxial connections, alongside a 25-pin DC connection for LNA bias at 50K and 5x 37-pin DC connections for the 4K LNA bias, TES bias, and SQUID flux ramp, per module \cite{Salatino20}.  The 4-6 GHz detector modules for the initial deployment will require 2 coax pairs each. 

\begin{figure}
\begin{center}
\includegraphics[width=0.4\textwidth]{figure/Readout_Chain/AliCPT_Readout_VJ_Plate.jpg}
\end{center}
\caption{The cryostat readout feedthrough panel that the warm readout electronics will interface with.  4 panels are needed for the final 19 module deployment, each capable of reading up to 5 detector modules.}\label{fig:Readout_Feedthrough}
\end{figure}
